Global-Position Tracking Control of 3-D Bipedal Walking via Virtual Constraint Design and Multiple Lyapunov Analysis

A safety-critical measure of legged locomotion performance is a robot's ability to track its desired time-varying position trajectory in an environment, which is herein termed as "global-position tracking". This paper introduces a nonlinear control approach that achieves asymptotic global-position tracking for three-dimensional (3-D) bipedal robot walking. Designing a global-position tracking controller presents a challenging problem due to the complex hybrid robot model and the time-varying desired global-position trajectory. Towards tackling this problem, the first main contribution is the construction of impact invariance to ensure all desired trajectories respect the foot-landing impact dynamics, which is a necessary condition for realizing asymptotic tracking of hybrid walking systems. Thanks to their independence of the desired global position, these conditions can be exploited to decouple the higher-level planning of the global position and the lower-level planning of the remaining trajectories, thereby greatly alleviating the computational burden of motion planning. The second main contribution is the Lyapunov-based stability analysis of the hybrid closed-loop system, which produces sufficient conditions to guide the controller design for achieving asymptotic global-position tracking during fully actuated walking. Simulations and experiments on a 3-D bipedal robot with twenty revolute joints confirm the validity of the proposed control approach in guaranteeing accurate tracking.

==> excess.tex <==
    % both the produced virtual constraints and 
    % to generate virtual constraints that guarantee 
    % that can be used in full-body trajectory generation to ensure
    % the planning of virtual constraints that ensures
    % to ensure 
    % both the produced virtual constraints and the 
    % the complete set of desired trajectories (i.e., the produced virtual constraints as well as the desired global-position trajectory) respect the impact dynamics, given any arbitrary global-position trajectories provided by a higher-level planner.
    % the complete set of desired motions (i.e., the desired functions produced by the virtual constraints as well as the desired global-position trajectory) respects the impact dynamics under any arbitrary global-position trajectories provided by a higher-level planner.}
    % \item[i)] \YanMod{Providing a set of constructive conditions that can be used as an equality constraint in the planning of virtual constraints, so as to ensure the complete set of desired motions (i.e., the desired functions defined by the virtual constraints and the desired global-position trajectory) respects the impact dynamics under any arbitrary global-position trajectories provided by a higher-level planner.}
% 	\item[i)] \YanMod{Providing a set of constructive conditions that can be used as an equality constraint to enforce impact dynamics in the planning of virtual constraints.
% 	method of designing virtual constraints that can be used to guarantee the full-order desired trajectories (i.e., functions that define the virtual constraints and the desired global-position trajectory specified by a high-level planner) will respect impact dynamics while helping to reduce the computational burden of trajectory generation.}
	%V1:
    % \item[i)] \YanMod{Providing a constructive method of designing virtual constraints that can be used to guarantee the full-order desired trajectories (i.e., functions that define the virtual constraints and the desired global-position trajectory specified by a high-level planner) will respect impact dynamics while helping to reduce the computational burden of trajectory generation.}
% 	\YanMod{Need to tie with global-position trajectories.. Need to be specific about and highlight HOW it reduces the burden...}
%	that addresses the nonlinear coupling of the robot's heading and lateral motions during 3-D walking and 
%	for producing desired motions respecting impact dynamics.
	%The virtual constraints produced meet a necessary condition required to achieve asymptotic global-position tracking under the condition that the robot's lateral foot placement to the walking direction is at the desired location. 
%	The virtual constraints produced meet a necessary condition required to achieve asymptotic global-position tracking
%	under certain lateral foot-placement condition. 
%	\textcolor{red}{This method can be used to greatly reduce the computational load in the generation of desired motions because it does not explicitly reply on the given desired global-position trajectory.}
%	Furthermore, since the virtual constraints produced only depend on the robot's actual posture, the robot's actual and desired motions will always simultaneously jump, thus eliminating the issue of intermittent tracking-error jumps.

% , and instead often planned as a smooth position trajectory in the world frame.
% Yet, the other desired trajectories for the full-order model are still free to be designed, for example, they can be chosen as virtual constraints.
% Thus, one way to enforce the impact dynamics in trajectory generation is to design virtual constraints such that both them and the desired global-position trajectory agree with the impact dynamics of the full-order model.
%
% v1
% \YanRes{Yet, the desired global-position trajectories are often specified by the higher-level planner as \YanRes{nonperiodic functions} encoded by the global time (which monotonically evolves across all walking steps).}
% % v2
% \YanRes{In global-position tracking tasks, the desired global-position trajectories are often specified by the higher-level planner as \YanRes{nonperiodic functions} encoded by the global time (which monotonically evolves across all walking steps).
% \YanRes{
% Thus, the design of virtual constraints needs to ensure the prespecified GP trajectories also respect the impact dynamics. 
% Because XXXX
% }
% \YanMod{V1:
% Because
% they may not be \YanMod{explicitly} encoded by a phase variable that represents the local progress within a step and is thus reset at the beginning of each step,}
% % For this reason, 
% the existing virtual constraint design cannot be directly extended to ensure the desired global-position trajectory respects the impact dynamics.}
% \YanMod{R2: This comment needs to be carefully revised. It does not seem to catch the real, basic reason why the existing design of virtual constraints cannot be used for global-position tracking control. What specific aspects of global position trajectory are not compatible with the existing methods? Is it because of periodicity? Or??}.
% V3:
% \YanRes{Yet, these methods mainly focus on the robot's joint angles and global velocities while the global position trajectory also depends on the absolute stance-foot position.
% Thus, it remains unclear how to design virtual constraints for global-position tracking control.}
% remains an underexplored problem, because 
% because they only consider joint positions and motions but a robot's global position trajectory also depends on stance-foot position.
% % V2:
% Yet, it remains unclear how to design virtual constraints for global-position tracking control because they only consider joint positions and motions but a robot's global position trajectory also depends on stance-foot position.
%V1:
% However, these methods are not suitable for global-position tracking control because they only consider joint positions and motions but a robot's global position trajectory also depends on stance-foot position.
%However, these methods are not suitable for global-position tracking as they cannot guarantee that the desired motions generated will respect impact dynamics during tasks of global-position tracking.
% \YanMod{Tone down the criticism while being fair. DONE for R1.}
% \YanMod{Need to introduce the concept of virtual constraints and impact invariance. Need to point out that HZD includes a virtual constraints design method that can satisfy the impact invariance condition.}



% - - - - - 

% V2:
% \YanRes{In this study, we choose the first set of desired position trajectories to be the reference global-position trajectory, and assume that they have been specified by a high-level path planner. 
% % The corresponding trajectory tracking errors are mathematically defined next. 
% }

% In real-world applications of robot locomotion, a path planner often provides the following desired global motions:
% \begin{enumerate}
% 	\item[a)] The center line $\Gamma_d$ of the desired global path.
% 	\item[b)] The desired smooth position trajectory along $\Gamma_d$.
% \end{enumerate}


% For simplicity and without loss of generality \YanMod{this phrase is used twice}, {the center line $\Gamma_d$} is specified as the $X_w$-axis of the world reference frame; i.e.,
% $
% \Gamma_d = \{(x_b,y_b) \in \mathbb{R}^2:  y_b =  0  \}.
% \label{Gamma}
% $
% %
% Let $x_d(t)$ be the desired smooth position trajectory along $\Gamma_d$.
% {
% 	Then, the global-position tracking error along $\Gamma_d$ is defined as
% 	$
% 	\bar{x}_b (\bq)-(x_{d}(t) - x_{st} )
% 	$.
% }

% - - - - 

% In real-world applications of robot locomotion, a path planner often provides the following desired global motions:
% \begin{enumerate}
% 	\item[a)] The center line $\Gamma_d$ of the desired global path.
% 	\item[b)] The desired smooth position trajectory along $\Gamma_d$.
% \end{enumerate}
% %The horizontal global motion specified by the path planner includes: a) the center line $\Gamma_d$ of the desired global path and b) the desired position trajectory along $\Gamma_d$.
% In this study, it is assumed that these desired motions have been specified by a higher-level planner.

% %Because this study focuses on flat-surface walking, it is assumed that the path planner (i.e., Level 2 in Fig.~\ref{fig-3levels}) specifies the global motion projected on the walking surface.

% % provides the desired horizontal global-position trajectory

% The horizontal components of the {base} position are:
% \begin{equation}
% 	x_b = x_{st} + \bar{x}_b (\bq)~\text{and}~
% 	y_b =y_{st} + \bar{y}_b (\bq),
% \end{equation}
% where 
% $ \bar{x}_b  : Q \rightarrow Q_x \subset \mathbb{R}$ and $ \bar{y}_b: Q \rightarrow Q_y \subset \mathbb{R}$ represent the $x$- and $y$-coordinates of the base position relative to the stance foot, respectively,
% and
% $(x_{st},y_{st},0)$ denotes the stance-foot position in $\Sigma_{X_w Y_w Z_w}$.


% For simplicity and without loss of generality, single-direction walking on horizontal flat surfaces is considered.
% \YanMod{For discussion: how to extend to walking with a changing direction.}

% Without loss of generality, a biped's {base} (e.g., chest) position $(x_b,y_b,z_b)$ in the world frame $\Sigma_{X_w Y_w Z_w}$ is chosen to represent its global position.


% For simplicity and without loss of generality \YanMod{this phrase is used twice}, {the center line $\Gamma_d$} is specified as the $X_w$-axis of the world reference frame; i.e.,
% $
% \Gamma_d = \{(x_b,y_b) \in \mathbb{R}^2:  y_b =  0  \}.
% \label{Gamma}
% $
% %
% Let $x_d(t)$ be the desired smooth position trajectory along $\Gamma_d$.
% {
% 	Then, the global-position tracking error along $\Gamma_d$ is defined as
% 	$
% 	\bar{x}_b (\bq)-(x_{d}(t) - x_{st} )
% 	$.
% }



% \subsection{Webots Simulations}

% {To implement the proposed controller on a physical OP3 robot, the ROS package ($op3\_manager$) developed by OP3's manufacturer was used in the experiments.}
% One controller implementation limitation of OP3 is that it does not allow users to access the output torques of joint motors when the ROS package is used for controller implementation.
% Instead, users can only send desired joint-position trajectories to individual joints and specify the PD gains of OP3's default joint controllers.
% %on \Todo{a scale of one to ten with one being the slowest and ten the fastest}. 
% This hardware limitation is common for today's bipedal humanoid robots~\cite{ames2012dynamically}.
% As the proposed control law in Eq.~\eqref{control-law} is a torque command, this hardware limitation prevents direct implementation of the proposed control law on OP3. 
% Thus, a controller implementation procedure is introduced to adapt the proposed control law for its implementation on the robot. 

% To gain preliminary insights into the effectiveness of the proposed controller implementation procedure,
% a Webots simulator is used to simulate a 3-D realistic robot model that closely emulates OP3's graphical, physical, and dynamical properties including its limited actuator accessibility.
%~\cite{webot1} 

% Since OP3's default joint controllers only allow users to send desired joint-position trajectories to individual joints, the proposed controller implementation procedure includes: a) to generate the desired position trajectory for individual joints $\mathbf{q}_d(t)$ and b) to send the desired trajectory to the default position controllers of the corresponding joints.
% The overall steps of this procedure are summarized as follows:
% \begin{itemize}
% 	\item[Step 1:] At the time step $t$, the nominal phase variable is computed as $\theta_d:=x_d(t)-x_{st}$. 
% 	\item[Step 2:] The desired joint position $\mathbf{q}_d(t)$ is computed by solving inverse kinematics.
% 	%	, i.e., $\mathbf{h}_c(\mathbf{q}_d(t)) - \mathbf{h}_d(t,\theta_d) =\mathbf{0}$.
% 	\item[Step 3:] $\mathbf{q}_d$(t) is fed into the joint controllers, which emulate the default joint controllers of a physical OP3 robot.
% \end{itemize}
% {A flow chart of the procedue is shown in Fig.~\ref{flow}.}
%\begin{itemize}
%	\item[Step 1:] At the time step $T$, the phase variable is computed as $\theta:=x_b(t)-x_{st}$. 
%	\item[Step 2:] The desired joint position $\mathbf{q}_d(t)$ is computed by solving $\mathbf{h}_c(\mathbf{q}_d(t)) - \mathbf{h}_d(t,\theta) =\mathbf{0}$.
%	\item[Step 3:] $\mathbf{q}_d$(t) is fed into the joint controllers, which emulate the default joint controllers of a physical \YanMod{OP3} robot.
%\end{itemize}

%Besides different controllers, the two simulators adopt different dynamic models of OP3.
% Due to the discrepancies in the implemented controllers and robot models, Webots simulations show a nonzero steady-state tracking error instead of asymptotic tracking as demonstrated in MATLAB simulation results.
% However, the bounded, relatively small tracking error obtained in Webots simulations indicates the effectiveness of the proposed controller implementation procedure in guaranteeing reliable trajectory tracking in the presence of robot hardware limitations and modeling errors.

% \subsection{Experiments}

% This subsection presents the experimental validation of the proposed control approach on a physical OP3 robot.
% The controller implementation procedure validated through Webots simulations is utilized to guide the experiments.

%\textcolor{red}{Add Youtube link.}


%\Todo{The details of the experimental controller implementation is shown in XXX.}





%\textcolor{blue}{Experiment results are shown in Figs.~\ref{fig5} and~\ref{fig6}.}
%Experimental results of the adapted control approach are given in Figs.~\ref{fig5} \YanMod{and~\ref{fig6}}. 
%\textcolor{blue}{The desired position trjectory along $\Gamma_d$$x_d(t)=0.044t-0.03$~m}




%Figure~\ref{fig5} (a) shows the global-position tracking results along $\Gamma_d$, and Fig.~\ref{fig5} (b) shows the global-path tracking results.


%	The comparison highlights the necessity of explicitly addressing uncertainties in the controller design, which is disucssed in Secition VII.}
%To enhance tracking performance for real-world robot operations, we will explicitly address the robustness issues caused by uncertainties in our future work, which is disucssed in Secition VII.

%For example, the robot's stance foot slighly slipped on the floor during the walking experiments, causing a mild violation of the theoretical modeling assumption as stated in Section II.

%The adapted controller cannot exactly realize zero steady-state tracking error mainly \YanMod{for two reasons: 1)} the OP3 robot's default individual joint controllers regulate joint positions without compensating for the nonlinear dynamic coupling among different joints} and \YanMod{2) uncertainties such as modeling errors and walking surface irregularity exist.} 
%However, reliable trajectory tracking can still be realized because the \YanMod{OP3} robot's default controllers can produce a reasonably fast continuous-phase convergence rate.

%Another reason is that the moderate uncertainties in these experiments can be mitigated by the inherent robustness of feedback control.
%\Todo{Indeed,
%The robot's stance foot slips significantly while walking on the tiled floor, thus resulting in a larger steady-state tracking error than that on the cemented floor. 
%The foot slippage can be clearly observed in the video as well. (Should I mention the video in the paper???)
%}
%\YanMod{Experiment results of OP3 walking on two common walking surfaces, i.e., tiled and cemented surfaces, are shown in Figs.~\ref{fig5} \YanMod{and~\ref{fig6}}.
%These figures show that a bounded steady-state tracking error can be realized despite hardware implementation imperfections.





%of $\Gamma_d$ and the desired position trajectory along $\Gamma_d$ 

%as shown in Figs.~\ref{fig6} (a) and (b)
%The concept of impact invariance was first introduced within the HZD framework, along with a systematic method of impact invariance construction (see Theorem 4 in~\cite{westervelt2003hybrid}). The concept was later on termed as ``impact invariance''~\cite{morris2009hybrid}.
%%The initial construction method consists of formulating the condition into an equality constraint and enforcing it in trajectory generation, thus producing desired trajectories that respect impact invariance.
%%{grizzle2001asymptotically,westervelt2003hybrid,morris2009hybrid}
%The HZD construction method cannot be used for the design of global-position tracking controllers because a robot's global position depends on both stance-foot and joint positions but the HZD method only considers joint positions.

%We have previously introduced a construction method that considers both stance-foot and joint positions for global-positon tracking control during 2-D walking~\cite{gu2017exponential}.
%The method cannot be used for 3-D walking because it does not explicitly address the inherent nonlinear coupling of a robot's global motion on a 2-D walking surface.
%This study extends our previous construction of impact invariance from 2-D to 3-D walking by explicitly addressing the nonlinear coupling. 
%Our stability analysis then provides sufficient conditions under which the proposed controller design provably guarantees the satisfaction of the stance-foot position condition at the steady state, as will be explained in Section V.

%\textcolor{orange}{The concept of impact invariance construction was first introduced within the HZD framework}~\cite{westervelt2003hybrid}.\Todo{Theorem 4 of 2003 TAC paper.}
%\textcolor{orange}{Later on, the concept is termed as ``impact invariance construction''}~\cite{morris2009hybrid}.
%\textcolor{blue}{OK!}

%The output function $\by$ and its derivative $\dot{\by}$ are {\it impact invariant} if the following condition is satisfied: $\by^+=\bzero$ and $\dot{\by}^+=\bzero$ automatically hold when $\by^-=\bzero$ and $\dot{\by}^-=\bzero$.

%\textcolor{orange}{
%	This impact invariance condition essentially requires that the reference trajectory should respect the robot's impact dynamics.
%	The robot cannot be directly controlled during impact events due to their infinitesimal period of duration.
%	Therefore, if the reference trajectory does not respect the impact dynamics, it may not be feasible for the robot's actual state to converge to the reference motion at the steady state. }
%\textcolor{blue}{OK!}

%\vspace{0in}
%\begin{figure}[h]
%	\centering
%	\includegraphics[width=0.8\linewidth]{fig/0Tk-3.png}%0Tk-1
%	\caption{
%		An illustration of the actual $k^{th}$ and $k+1^{th}$ steps ($k \in \{1,2,... \}$).
%		The actual $k^{th}$ step begins at $t=T_{k-1}^+$ and ends at $t=T_{k}^-$.
%		The actual $k^{th}$ swing-foot landing occurs at $t=T_{k}^-$.  
%		\YanMod{Consider deleting this plot.}
%	}
%	\label{fig-Tk}
%\end{figure}
%\vspace{0in}



% The impact invariance of the This is valid because, if $\bar{x}_b (\bq)-(s_{d}(t) - x_{st} )=0$ and theta does not jump, then y+=0 automatically holds as thetad does not jump as well.
% The condition that ensures the dtheta does not jump when evolving along the desired state trajectories is given below (\YanMod{B2}):
% \YanMod{R3: add the new impact condition here. Also, highlight its advantages as outlined.}

% Furthermore, this condition can be translated into a condition solely on the robot's desired posture just before a jump; that is:

% XXX



% \subsection{Conditional Impact Invariance Construction}

% \YanMod{Why do we need to guarantee the uniqueness/existence for conditional impact invariance construction??}
% \YanMod{How previous impact invariance construction works.}
% \YanMod{revise this paragraph.}


% \YanMod{Briefly summarize how ours works and it is different from previous work.
% Point out we need to explicitly consider the timing, and use it to introduce the next paragraph.
% }

% \YanMod{Why do we need this assumption? What does it have to do with Theorem 9? What is the underlying design choice? What is the rationale of this design choice?}

% \YanRes{To ensure that the control authority of the robot is fully exploited to command $n$ independent control variables, we choose the control variables ${\bh}_c$ to be a linear independent set of variables. The following assumption mathematically summarizes}

% \begin{assum}
% [\textbf{Invertible Jacobian of Control Variables}]
% 	%	Define
% 	%	$$
% 	%	\bH_v (\bq):= \begin{bmatrix}
% 	%		\frac{ d \bm \phi_c }{ d \bq  }^T (\bq) ~
% 	%		\frac{ d \bar{x}_b }{ d \bq  }^T (\bq) ~
% 	%		\frac{ d \bar{y}_b }{ d \bq  }^T (\bq)
% 	%	\end{bmatrix}^T.
% 	%$$
% 	{
% 		Define the Jacobian matrix of the control variable ${\bh}_c$ as
% 		$
% 		\bJ_h (\bq):= 
% 		\frac{ d {\bh}_c }{ d \bq  } (\bq)
% 		=
% 		\begin{bmatrix}
% 			\frac{ d \bar{x}_b }{ d \bq  }^T (\bq),
% 			\frac{ d \bar{y}_b }{ d \bq  }^T (\bq),
% 			\frac{ d \bm \phi_c }{ d \bq  }^T (\bq)
% 		\end{bmatrix}^T.
% 		$
% 	}
% 	$\bJ_h(\bq)$ is locally invertible within a small neighborhood about $\bq^*$.
% 	\label{assume-inv}
% \end{assum}
% Assumption~\ref{assume-inv} can be met by choosing $\bm \phi_c$ to be independent from $\bar{x}_b$ and $\bar{y}_b$.

% \YanMod{Why do we need this assumption? What does it have to do with Theorem 9? What is the underlying design choice? What is the rationale of this design choice?}
% \begin{assum}
% 	%	Define
% 	%	$$
% 	%	\bH_v (\bq):= \begin{bmatrix}
% 	%		\frac{ d \bm \phi_c }{ d \bq  }^T (\bq) ~
% 	%		\frac{ d \bar{x}_b }{ d \bq  }^T (\bq) ~
% 	%		\frac{ d \bar{y}_b }{ d \bq  }^T (\bq)
% 	%	\end{bmatrix}^T.
% 	%$$
% 	{
% 		Define
% 		$
% 		\bH_v (\bq):= \begin{bmatrix}
% 			\frac{ d \bar{x}_b }{ d \bq  }^T (\bq) ~
% 			\frac{ d \bar{y}_b }{ d \bq  }^T (\bq)~
% 			\frac{ d \bm \phi_c }{ d \bq  }^T (\bq)
% 		\end{bmatrix}^T.
% 		$
% 	}
% 	Define $ \bq_0 :=  \bm \Delta_{q} (\bq^*)$ and $\theta_0 := \bar{x}_b(\bq_0).$
% 	$\bH_v(\bq)$ is locally invertible within a small neighborhood about $\bq^*$.
% 	\label{assume-inv}
% \end{assum}
% Assumption~\ref{assume-inv} can be met by choosing $\bm \phi_c$ to be independent from $\bar{x}_b$ and $\bar{y}_b$.%	The assumption (A2) holds during forward walking.
% \YanMod{Incorporate this sentence into the assumption.}
% \YanMod{Provide intuitive explanation of this assumption.}


    % \YanRes{This reduces the computational load of virtual constraint generation in the presence of nonperiodic desired global-position trajectories}.
    % \YanMod{still need to tweak a bit.}
    % \item[i)] 
    % % \YanMod{
    % Providing a set of 
    % % constructive conditions that can be used as an 
    % equality constraints
    % that can be incorporated in a trajectory generator to produce \YanRes{virtual constraints}
    % % \YanRes{the additional desired full-body trajectories} 
    % that respect the impact dynamics.
    % Furthermore, enforcing the proposed equality constraints automatically ensures any arbitrary global-position trajectories provided by a higher-level planner will respect the impact dynamics. \YanRes{This reduces the computational load of virtual constraint generation in the presence of nonperiodic desired global-position trajectories}.
    % \YanMod{still need to tweak a bit.}
    % The attractive feature ensures to ensure
    % the complete set of desired trajectories (i.e., the produced virtual constraints as well as the desired global-position trajectory) respect the impact dynamics, given any arbitrary global-position trajectories provided by a higher-level planner.
    % that can be used in the planning of virtual constraints to ensure
    % the complete set of desired trajectories (i.e., the produced virtual constraints as well as the desired global-position trajectory) respect the impact dynamics, given any arbitrary global-position trajectories provided by a higher-level planner.
    
    
    %	To our best knowledge, this is the first time that trajectory tracking control that explicitly addresses hybrid walking dynamics has been realized on physical robot platforms.
%	Results of comparative experiments show the proposed trajectory tracking control law achieves a much higher tracking accuracy than orbit tracking control.


%	Besides the closed-loop tracking performance, these conditions also guarantee that the foot-placement condition underlying the proposed virtual constraint design is satisfied at the steady state; that is, the robot's lateral foot placement asymptotically converges to its desired location. 
%	Also, they ensure that the actual impact timings converge to their desired values at the steady state. 

% Towards tackling the challenges in achieving asymptotic global-position tracking for 3-D fully actuated bipedal walking, 
% this study focuses on:
% a) \YanMod{deriving design the remaining desired full-body motions such that} \YanRes{the complete set of desired trajectories} respect impact dynamics and b) to derive a control law that provably achieves asymptotic global-position tracking during 3-D bipedal walking by explicitly handling the hybrid robot dynamics.
% , 

% Fig.~\ref{fig-3levels} shows the three levels of a representative autonomous robot locomotion system~\cite{manchester2011stable}.
% This study focuses on Level 3: Locomotion Control.

%The objective of this study is to derive a control approach that explicitly addresses the hybrid walking dynamics for provably realizing asymptotic global-position tracking during fully actuated 3-D bipedal robotic walking.
%The goal of this study is to tackle these two challenges for 3-D fully actuated bipedal walking.
%To provide the context of this study, it is assumed that the desired heading direction and the desired global-position trajectory in that direction has been provided by a higher-level path planner.
%Thus, the focus of this study is: a) to design the remaining desired motions such that the complete set of desired motions respect impact dynamics and b) to derive a control law based on formal stability analysis of the hybrid closed-loop system for achieving asymptotic global-position tracking during 3-D bipedal walking.
%Deriving such a control approach is still an underexplored problem as reviewed next.


%Thus, the focus of this study is on deriving a control approach that explicitly addresses hybrid robot dynamics for provably achieving asymptotic global-position tracking during 3-D bipedal walking, which remains an underexplored control problem as reviewed next.
%Thus, the focus of this study is on deriving a control approach that a) produces the remaining desired motions such that the complete set of desired motions respect impact dynamics and b) explicitly addresses hybrid robot dynamics for provably achieving asymptotic global-position tracking during 3-D bipedal walking.
%Deriving such a control approach is still an underexplored problem as reviewed next.



%To achieve asymptotic global-position tracking for 3-D fully actuated bipedal robotic walking,
%\textcolor{blue}{our proposed control approach has three main components:
%	a) a state-feedback controller design for realizing asymptotic trajectory tracking during {\it continuous} phases;
%	b) a constructive method of synthesizing virtual constraints based on the proposed construction of conditional impact invariance;
%%	for satisfying a necessary condition required to achieve asymptotic trajectory tracking for the overall hybrid process;
%%	for producing desired motions that respect jump dynamics;
%	and c) Lyapunov-based stability analysis of the hybrid closed-loop system that examines the convergence of the global position in the nonlinearly coupled heading and lateral directions.
%%	produces sufficient conditions to guide the design of the continuous-phase control law
%%	 for guaranteeing asymptotic trajectory tracking for the overall {\it hybrid} control system.
%	}


%the objectives of this study are: a) to design desired motions that respect impact dynamics without causing a heavy computational burden and b) to derive a control law based on formal stability analysis of the hybrid closed-loop system for achieving asymptotic global-position tracking during 3-D bipedal walking.
%To achieve asymptotic global-position tracking for 3-D fully actuated bipedal robotic walking,

%A discrete-time system has been constructed and analyzed based on Lyapunov theory to provide sufficient conditions that guarantee the tracking performance of linear fully actuated systems~\cite{menini2001asymptotic}. 
%Yet, this method does not explicitly address the intermittent jumps of tracking errors induced by the mismatch in the jump timings between the actual and the desired state trajectories.
%Recent studies have focused on resolving the jump-time mismatch issue 
%by introducing novel tracking error notions that essentially adjust the jump timings of the desired state trajectory to match those of the actual one~\cite{biemond2012tracking,forni2013follow,rijnen2016hybrid,rijnen2017control}.
%With the aligned jump timings, a 
%V1:
% \YanMod{However, the evolution of the Lyapunov function across nonlinear state-triggered jumps,
% which are an inherent feature of robot walking dynamics, 
% is not explicitly analyzed in these previous studies.
% V1
% However, the evolution of the Lyapunov function across nonlinear state-triggered jumps,
% which are an inherent feature of robot walking dynamics, 
% is not explicitly analyzed in these previous studies.
% Thus, it is not yet clear how to use these previous trajectory tracking control methods to directly inform the global-position tracking controller design for walking robots that possess highly nonlinear jumps.}
%V2:
% (In particular, we will analyze the effects of nonlinear state-triggered jumps in the evolution of Lyapnov functions.)}
% \YanMod{(Tone down the criticism while being fair. These attacks are too generic and need to be specific. Done for R1.) R2: Perhaps point out what is particularly challenging with the extension.}


% \YanRes{
% In global-position tracking tasks, the desired full-body trajectories include the desired global-position trajectories, which are often supplied by the higher-level planner.} 
% Because they are often planned as continuous trajectories instead of explicitly agreeing with the impact dynamics, the generation of the remaining full-body desired trajectories (e.g., desired functions associated with virtual constraints) need to ensure the desired global-position trajectory also respects the impact dynamics in addition to their own compatibility.
% Yet, because the desired global-position trajectories are often \YanRes{nonperiodic functions} encoded by a global phase variable (which monotonically evolves across all walking steps), 
% the existing virtual constraint design cannot be directly employed to ensure the desired global-position trajectory respects the impact dynamics.
% }

% they cannot be designed or represented through virtual constraints encoded by a local phase variable.
% \YanRes{They are often pre-specified by the higher-level planner as \YanRes{nonperiodic functions} encoded by a global phase variable (which monotonically evolves across all walking steps).
% Thus, they cannot be designed or represented through virtual constraints encoded by a local phase variable.
% , or altered for safety purposes such as obstacle avoidance.
% Also, they are often not planned to explicitly agree with the impact dynamics, which means that the generation of the remaining full-body desired trajectories need to ensure the desired global-position trajectory also respects the impact dynamics in addition to their own compatibility.
% For these reasons, 


%V1
% \YanRes{They are often pre-specified by the higher-level planner as \YanRes{nonperiodic functions} encoded by a global phase variable (which monotonically evolves across all walking steps).
% Thus, they cannot be designed or represented through virtual constraints encoded by a local phase variable.
% % , or altered for safety purposes such as obstacle avoidance.
% Also, they are often not planned to explicitly agree with the impact dynamics, which means that the generation of the remaining full-body desired trajectories need to ensure the desired global-position trajectory also respects the impact dynamics in addition to their own compatibility.
% For these reasons, the existing virtual constraint design cannot be directly extended to ensure the desired global-position trajectory respects the impact dynamics.
% }


%Second, a controller capable of reliably tracking a time-varying global-position trajectory can result in a hybrid, nonlinear, and time-varying closed-loop walking control system, whose stability and tracking performance will be complicated to analyze.
%
%\textcolor{red}{There are two specific challenges associated with the global-position tracking control problem for bipedal robotic walking. First, the desired motions that a robot should reliable track, including the desired global-position trajectory, need to be designed to respect the jump dynamics for achieving asymptotic trajectory tracking for hybrid systems with jumps. Yet, due to the high complexity of walking dynamics, the computational load of such design can be overly high for enabling online planning. Second, a controller capable of reliably tracking a time-varying global-position trajectory can result in a hybrid, nonlinear, and time-varying closed-loop walking control system, whose stability and tracking performance will be complicated to analyze.}

%To date, it remains an underexplored problem to derive control laws that explicitly address hybrid robot dynamics for provably achieve asymptotic global-position tracking during 3-D bipedal walking. 


% \YanMod{
% Towards tackling these two challenges for 3-D fully actuated bipedal walking, the objectives of this study are: a) to design desired motions that respect impact dynamics without causing a heavy computational burden and b) to derive a control law based on formal stability analysis of the hybrid closed-loop system for achieving asymptotic global-position tracking during 3-D bipedal walking.
% Deriving such a control approach is still an underexplored problem as reviewed next.
% Previous work related to this study is reviewed next.
% To provide the context of this study, it is assumed that the robot's desired heading direction and the desired global-position trajectory in that direction has been provided by a higher-level path planner.
% Thus, the focus of this study is: a) to design the remaining desired motions such that the complete set of desired motions respect impact dynamics and b) to derive a control law based on formal stability analysis of the hybrid closed-loop system for achieving asymptotic global-position tracking during 3-D bipedal walking.
% Deriving such a control approach is still an underexplored problem as reviewed next.
% }


% \YanMod{Revise this paragraph.}
% The goal of this study is to create a control approach that explicitly addresses the hybrid walking dynamics of bipedal robots for achieving reliable global-position tracking control.

% Deriving such a control approach is still an underexplored problem as reviewed next.

% \vspace{0in}
% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=1\linewidth]{fig/003levels-1.png} %03levels-2
% 	\caption{
% 		A representative autonomous robot locomotion system. This study addresses Level 3: Locomotion Control. 
%  		\YanMod{consider deleting this figure. 
% % 		Refer to this figure.
% 		}
% 	}
% 	\label{fig-3levels}
% \end{figure}
%\vspace{-0.1in}

% \subsection{Related Work}


% \YanMod{This is true when input-output linearizing controller is used..
% Perhaps we should introduce I-O linearizing controller first and then introduce this necessary constraints. Wait.. Actually, even for optimal control, respecting the impact invariance condition is necessary... Essentially, this is needed to ensure the desired motion respects the impact dynamics. 
% }
% This is essentially because the impact dynamics cannot be directly controlled due to their infinitesimally short periods of duration.
%V2:
% In particular, the robot's desired motions need to be designed to respect the impact dynamics (i.e., the jumps) for achieving asymptotic tracking.
% This is because bipedal walking dynamics are inherently hybrid involving state-triggered jumps, e.g., sudden jumps in joint velocities upon a foot-landing impact~\cite{golliday1977approach, hurmuzlu1986role, goswami1997limit, westervelt2007feedback}, which cannot be directly controlled due to their infinitesimally short periods of duration.
%V0:
% Bipedal walking dynamics are inherently hybrid involving state-triggered jumps, e.g., sudden jumps in joint velocities upon a foot-landing impact~\cite{golliday1977approach, hurmuzlu1986role, goswami1997limit, westervelt2007feedback}. 
% Because these jumps cannot be directly controlled due to their infinitesimally short periods of duration, the robot's desired motions need to be designed to respect the impact dynamics (i.e., the jumps) for achieving asymptotic tracking.


%%The accuracy of global-position tracking relies on the underlying control approaches, but the controller 
%Achieving reliable global-position tracking presents substantial controller design challenges mainly due to the high complexity of bipedal walking dynamics.
%First, bipedal robotic walking is inherently a hybrid dynamical process involving state-triggered jumps, e.g., sudden jumps in joint velocities upon a swing-foot landing~\cite{golliday1977approach, hurmuzlu1986role, goswami1997limit, westervelt2007feedback}. 
%These jumps cannot be directly controlled due to their infinitesimally short periods of duration.
%Second, a controller capable of reliably tracking a time-varying global-position trajectory can result in a hybrid, nonlinear, and time-varying closed-loop walking control system, whose stability and tracking performance will be complicated to analyze.
%
%\textcolor{red}{There are two specific challenges associated with the global-position tracking control problem for bipedal robotic walking. First, the desired motions that a robot should reliable track, including the desired global-position trajectory, need to be designed to respect the jump dynamics for achieving asymptotic trajectory tracking for hybrid systems with jumps. Yet, due to the high complexity of walking dynamics, the computational load of such design can be overly high for enabling online planning. Second, a controller capable of reliably tracking a time-varying global-position trajectory can result in a hybrid, nonlinear, and time-varying closed-loop walking control system, whose stability and tracking performance will be complicated to analyze.}

% \YanMod{R3: perhaps move ZMP here, and then explain the complexity in achieving 3D GPT for the hybrid model.}
% \YanMod{R3: justify why we consider a hybrid model.}

% \subsection{Related Work on Bipedal Walking Control}
% To achieve accurate global-position tracking, the Zero-Moment-Point (ZMP) control approach has been introduced based on the ZMP balance criterion and the continuous-time dynamics of bipedal walking~\cite{vukobratovic2001zero,kajita2003biped,kim2006experimental}.
% \YanRes{The ZMP approach focuses on the continuous-time dynamics of a walking robot by ignoring the jumps in a robot's joint velocities caused by foot-landing impacts.}
% \YanMod{Is this accurate? Besides velocity jumps, are there other behaviors that can cause hybrid dynamics? Maybe I can just delete??}

% Achieving reliable global-position tracking presents substantial controller design challenges mainly due to the high complexity of bipedal walking dynamics, which are inherently hybrid involving continuous-time dynamics (e.g., foot swinging) and state-triggered jumps (e.g., sudden jumps in joint velocities upon a foot-landing impact)~\cite{golliday1977approach, hurmuzlu1986role, goswami1997limit, westervelt2007feedback}.


% our future work on extending the proposed controller design for enabling global-position tracking over complex terrains as well as for improving robustness against uncertainties.}

% This study has introduced a global-position tracking controller that explicitly addresses the hybrid model of 3-D fully actuated bipedal robot walking.
% The first main contribution of the study is the
% extension of

%
% \YanMod{Analogous to the previous method~\cite{westervelt2003hybrid}, the condition is only directly imposed on the phase variable encoding the virtual constraints instead of the full DOFs of the robot, thus helping to reduce the computational load of motion planning.
%


% to enhance its performance.


% \YanMod{Highlight that the same set of virtual constraints is used for two different global-position trajectories, and yet the impact invaraince condition is still satisfied. }

% \begin{rem}
% 	\YanRes{
% % 	Corollary 16 indicates that the proposed controller design can ensure the robot's swing foot lands on the walking surface with the accurate timings.
% % 	The rationale of the proof is that the impact timing error $T_{k} - \tau_k$ is bounded above in norm by the norm of the state and thus asymptotically diminishes as the state is driven to zero.
% 	Note that}
% % 	In contrast to the proposed global-position tracking control, 
% 	an orbitally stabilizing controller cannot achieve the asymptotic tracking of the desired global position trajectories, as explained in Section~\ref{sec-related}.
% 	Accordingly \YanMod{why? done}, it cannot realize asymptotic convergence to the desired timing $\tau_k$ but can realize a finite final error for $T_k-\tau_k$. 
% % 	\YanMod{so what?}
% 	\YanMod{Tone down the criticism. Perhaps just call this a distinctive feature.. Or move this to the discussion section.}
% 	\YanMod{R3: we can add equation to illustrate this? didn't do it because it is not necessary.}
% \end{rem}







%, and \textcolor{brown}{using on-board sensors for state estimation.}



%\YanMod{Discuss the intermittent jump issue. Discuss the Lyapunov function design for multi-mode walking}


%\YanMod{Highlight that we don't have the intermittent jump issue thanks to the error design. as long as higher-level planners would provide smooth global motions as they typically do in real-world robot applications... as long as higher-level planners would provide smooth global motions as they typically do in real-world robot applications...}



%\subsection{\textcolor{blue}{Global-Position Tracking on 3-D Terrains}}


%
%\textcolor{blue}{Also, we will develop efficient trajectory generation methods for enabling online planning. Our recent study has shown that exploiting offline planning effort could significantly improve online planning efficiency for bipedal walking along a general-shaped path on flat surfaces~\cite{gao2019impact}. Our future work will extend this recent result to realize online motion planning of bipedal walking on a 3-D terrain.}

%\subsection{\textcolor{blue}{Robust Global-Position Tracking Control}}

%\textcolor{blue}{
%Another potential approach is to integrate the proposed controller design with a finite state machine that guides the switching among different controllers. For example, one of the controllers could be a ``recovery'' controller designed for regaining a robot's balance after a severe external push.} 



% full set of desired trajectories (i.e., the desired global-position trajectory supplied by the higher-level planner and the desired functions defining the planned virtual constraints) respect the impact dynamics. 
% The method produces conditions that can be imposed as equality constraints in the planning of virtual constraints, in order to ensure the full set of desired trajectories (i.e., the desired global-position trajectory supplied by the higher-level planner and the desired functions defining the planned virtual constraints) respect the impact dynamics. 
% In particular, any conditions produced hold under arbitrary  the desired global-position trajectory (e.g., supplied by a higher-level planner) yet it ensures all desired motions (including the GPT trajectories) are impact invariant.
% %
% The advantage is demonstrated through MATLAB and Webots simulation results.




%% Complete
% \YanRes{
% In global-position tracking tasks, the desired global position trajectories are often supplied by a higher-level planner without the impact map considered.
% Thus, the previous impact invariance construction cannot be directly placed on them for ensuring their compatibility with the impact dynamics.
% Also, because the virtual constraints encoded by a local phase variable and desired global-position trajectories are nonlinearly kinematically coupled in general, they affect each other's impact map.
% Thus, as the desired global position trajectory changes during real-world operations such as dynamic obstacle avoidance, the virtual constraints would need to be replanned in order to ensure they respect the impact dynamics. 
% The frequent demand in replanning the virtual constraints could cause a heavy computational burden especially during real-world tasks when the desired global position trajectory is nonperiodic due to online update.
% }

% \YanRes{
% Yet, because the desired global-position trajectories are often generated by the higher-level planner without the impact map considered, the previous impact invariance condition cannot be directly placed on the desired global-position trajectories through full-body trajectory generation to ensure they agree with the impact dynamics. 
% }
% \YanMod{So what?}
% \YanMod{However, the impact map of the global position and velocity are generally nonlinearly coupled with that of the virtual constraints, and thus the supply of the global position trajectory will generally affect the impact invariance of the virtal constraints (?? Not true.. We can also scale it...), and the impact invariance of the global position rtajctort needs to be ensured through the virtual constraint design. Thus, there is a need to plan the virtual constraints so that the desired global psoition and velocty trajectory also satisfy the impct map. the computational cost can be high the GPT may be nonperiodic and updated online during the task, which, without explicitly addressed, would result in frequent demands in virtual constraint replanning.}


% in order to ensure they respect the impact dynamics.
% they affect each other's impact map.
% Thus, as the desired global position trajectory changes during real-world operations such as dynamic obstacle avoidance, the virtual constraints would need to be replanned in order to ensure they respect the impact dynamics. 
% The frequent demand in replanning the virtual constraints could cause a heavy computational burden especially during real-world tasks when the desired global position trajectory is nonperiodic due to online update.


% Towards enabling provable global-position tracking for 2-D fully actuated bipedal robotic walking,
% we have previously extended the impact invariance construction of the HZD framework \YanMod{cite paper here} to explicitly incorporate a 2-D robot's global position~\cite{gu2016bipedal,gu2017exponential} \YanMod{Yuan's multi}.
% \YanMod{This design can be incorporated into the full-body trajectory generation to ensure the produced desired motions respect the impact dynamics.
% }
% Based on
% Lyapunov stability analysis, we have also derived sufficient conditions under which a continuous-phase control law provably achieves asymptotic global-position tracking associated with 2-D bipedal walking.


%introduces an orbitally stabilizing control method that drives a robot's state to converge to the periodic orbit corresponding to the desired motions.
%V2:%V1:
% Yet, the resulting orbitally stabilizing controller cannot drive the state to converge to a prespecified time-varying trajectory that resides in the orbit~\cite{khalil1996nonlinear}. % \YanMod{R2: This sentence does not explain what specific aspect of desired global-position trajectory that is not compatible with orbitally stabilizing control -- How about now?}.
% orbitally stabilizing control cannot {directly} guarantee asymptotic global-position tracking. 
% use the Poincar\'e section method to analyze the stability of a closed-loop system under global-position tracking control.
% \YanMod{Tone down the criticism while being fair. I need to think of another way to comment on HZD. Done for R1.}
%Thus
%{In fact, it is still not yet clear how to extend the orbitally stabilizing HZD method to achieve asymptotic trajectory tracking.}


%V3:
% \YanRes{The first main contribution of this study is a set of constructive conditions under which the desired full-body trajectories agree with the impact dynamics regardless of the desired global-position trajectory supplied by a higher-level planner.
% satisfy a necessary condition for realizing asymptotic trajectory tracking of hybrid walking systems.}
%V2:
% \YanRes{The first main contribution of this study is a set of constructive conditions under which the desired full-body trajectories agree with the impact dynamics and thus satisfy a necessary condition for realizing asymptotic trajectory tracking of hybrid walking systems.}
%V1:
% \YanRes{The first main contribution of this study is a set of constructive conditions under which the desired full-body trajectories satisfy a necessary condition for realizing asymptotic trajectory tracking of hybrid walking systems.}
\YanMod{too vague.}



% \YanRes{Corollary 16 indicates that the proposed controller design can ensure the robot's swing foot lands on the walking surface with the accurate timings.
% The rationale of the proof is that the impact timing error $T_{k} - \tau_k$ is bounded above in norm by the norm of the state and thus asymptotically diminishes as the state is driven to zero.}

% Theorem~\ref{theorem2} indicates that the lateral foot-placement condition underlying the proposed conditional impact invariance construction in Theorem~\ref{theorem 1} is indeed met at the steady state.
% Thus, the impact invariance of $\bx$, \YanRes{which is the necessary condition for asymptotic trajectory tracking,} is indeed satisified at the steady state; if $\bx(\tau_k^-) \rightarrow \bzero$ then $\bx(\tau_k^+)=\bm \Delta(\tau_k,\bzero) \rightarrow \bzero$ as $k \rightarrow \infty$.


% \YanMod{R3: Refer to eq. XX for the expression of V. done}
% \YanRes{The construction of $V(\bx)$ is given in Remark 13XX.}
% \YanMod{R3: What's the essence of having the foot placement convergence in the Lyapunov function??}
%

% To simplify the stability analysis using the proposed conditional impact invariance, which holds when $y_{st}=y_{std}$, we will explicitly analyze the convergence of $y_{st}$ to $y_{std}$.
% 	Thus, an augmented Lyapunov function candidate is constructed as

% The stability condition is derived based on the stability theory of the multiple Lyapunov functions~\cite{branicky1998multiple}, by which the hybrid dynamical system in Eq. XX is asymptotically stable if the Lyapunov function asymptotically converges during continuous phases and the jumps in the Lyapunov function just after all hybrid transitions are strictly decreasing.

% \YanMod{R3: add a black solid square here.}


% \YanMod{R3: give rationale for the convergence of the stance foot location.}

% To explicitly consider the effects of the convergence of the lateral foot placement on the system stability, 

% By the stability theory based on the construction of multiple Lyapunov functions~\cite{branicky1998multiple},

% \begin{rem}
% 	Corollary~\ref{cor1} indicates that the lateral foot-placement condition underlying the proposed conditional impact invariance construction in Theorem~\ref{theorem 1} is indeed met at the steady state.
	%	necessary condition for realizing asymptotic trajectory tracking, i.e., 
	%	Thus, the conditional impact invariance of $\bx$, is indeed met at the steady state; 
% 	Then, by Corollary~\ref{cor1} and Theorem~\ref{theorem 1}, if $\bx(\tau_k^-) \rightarrow \bzero$ then $\bx(\tau_k^+)=\bm \Delta(\tau_k,\bzero) \rightarrow \bzero$ as $k \rightarrow \infty$. 
% \end{rem}


% 	condition 
% % 	$y_{st} = y_{std}$ 
% 	underlying the proposed conditional impact invariance construction in Theorem~\ref{theorem 1} will indeed hold at the steady state; that is,
% 	$y_{st} \rightarrow y_{std}  ~ \mabox{as}~ t \rightarrow \infty.$
% % 	which indicates that if $\bx(\tau_k^-) \rightarrow \bzero$ then $\bx(\tau_k^+)=\bm \Delta(\tau_k,\bzero) \rightarrow \bzero$ as $k \rightarrow \infty$. 
% Finally, the actual impact timing $T_k$ will asymptotically converge to the desired timing $\tau_k$;
% 	that is, 
% 		$T_{k} \rightarrow \tau_k  ~ \mabox{as}~ k \rightarrow \infty.$
		
% 	Furthermore, the lateral foot-placement condition 
% % 	$y_{st} = y_{std}$ 
% 	underlying the proposed conditional impact invariance construction in Theorem~\ref{theorem 1} will indeed hold at the steady state; that is,
% 	$y_{st} \rightarrow y_{std}  ~ \mabox{as}~ t \rightarrow \infty.$
% % 	which indicates that if $\bx(\tau_k^-) \rightarrow \bzero$ then $\bx(\tau_k^+)=\bm \Delta(\tau_k,\bzero) \rightarrow \bzero$ as $k \rightarrow \infty$. 
% Finally, the actual impact timing $T_k$ will asymptotically converge to the desired timing $\tau_k$;
% 	that is, 
% 		$T_{k} \rightarrow \tau_k  ~ \mabox{as}~ k \rightarrow \infty.$
% 	\YanMod{R3: add equation for convergence of the stance foot location. done}


% 	This lower bound is given in Eq.~\eqref{c5-B} \YanMod{Talk about this equation without referring to it..}.
% 	While it is straightforward to choose the PD gains such that $\bA$ is Hurwitz, 
% 	to meet the conditions in Eq.~\eqref{c5-B} 

% respect impact dynamics and other necessary constraints.

% the OP3 robot should reliably track in simulations and experiments.
% \YanMod{R2: Point out what is the novelty here.. Direct application of previous planning method. Also, tie with the proposed virtual constraints construction.
% Explain why we need to do trajectory generation here.
% }

% 	Without loss of generality \YanMod{What do I exactly mean by ``without loss of generality''}, 
% 	\YanRes{As a legged robot's trunk typically oscillates about the walking path during walking,}

% \YanMod{R6: why bezier curves.}
%\YanMod{Are $\theta^+$ and $\theta^-$ used somewhere before Simulations?}

% Optimization techniques are utilized to generate the desired lateral base position $y_d$ and the desired function $\bm \phi_d$.



% \begin{figure}[t]
% 	\centering
% 	%	\includegraphics[width=0.8\linewidth]{fig/0MATLAB-B.png}%matlab_tracking_performance2
% 	\includegraphics[width=1\linewidth]{overleaf/fig/fig6_varing_speed_edited.png}%matlab_tracking_performance2
% 	\caption{
% 		{Global-position tracking results in MATLAB and Webots simulations with $x_d(t)=0.031t-0.015+0.015\sin(0.3t)-0.01\sin(0.8t)$~m.}
% 		\YanMod{Texts are two small. Too many colors. Lines are too thin.}
% 		}
% 	\label{fig2-varying}
% %	\vspace{-0.1in}
% \end{figure}


%\Todo{despite relatively large initial tracking errors (???). }
%\Todo{The initial tracking error is $x_b(0)-x_d(0)=3$~cm, which is approximately a half step length.}

% Figures~\ref{fig2} (a) and \ref{fig2-varying} (a) show the position tracking results of $s_d(t)$.
% ``$x_{bm}$'' represents the actual global-position trajectory along $\Gamma_d$, which asymptotically converges to $x_d(t)$ in both plots. 
% Figures~\ref{fig2} (b) and \ref{fig2-varying} (b) show the global-path tracking results. 
% {\it left foot (M)} and {\it right foot (M)} are the actual stance-foot positions, which indicate asymptotic tracking of the center line $\Gamma_d$ of the desired path.
% ``$x_{bw}$'' is the actual global-position trajectory along $\Gamma_d$ obtained in Webots simulations,
% and {\it left foot (W)} and {\it right foot (W)} are the actual stance-foot positions in Webots simulations.
% \YanMod{R6: some labels are off.}



% The initial tracking error of the desired position trajectory $s_d$ is $3$~cm, which is approximately $1/3$ of a nominal step length.


v% Due to the discrepancies in the implemented controllers and robot models, Webots simulations show a nonzero steady-state tracking error instead of asymptotic tracking.
% MATLAB results demonstrate that the proposed control law can drive the robot to 
% asymptotically converge to the desired position trajectory $s_d$ while moving along the center line $\Gamma_d$.
% Due to the discrepancies in the implemented controllers and robot models, Webots simulations show a nonzero steady-state tracking error instead of asymptotic tracking.
% as demonstrated in MATLAB simulation results.
% \YanMod{Both of them seem to be zero?}


% \begin{itemize}
%     \item [\textbf{Virtual constraint tracking accuracy.}]
% As shown in Fig.~\ref{fig4}, despite the relatively large initial tracking error, the proposed control law is capable of accurately enforcing the virtual constraints during 3-D fully actuated walking.
% % \YanMod{R3: add more words on interpreting the results.}
% % \YanMod{R4: Add Webots results here.}
% \end{itemize}


% \YanMod{R3: description of MATLAb results are missing...}
% \YanMod{R3: Initial tracking errors?}
% \YanMod{R3: why choose these control gains....e.g., we tune these gains to allow sufficiently fast continuous-phase convergence rate as requried in Theorem XXX ensure convergence...}% summarized as follows (Fig.~\ref{flow}).
% \begin{itemize}
% 	\item[Step 1:] At the time step $t$, the nominal phase variable is computed as $\theta_d:=s_d(t)-x_{st}$. 
% 	\item[Step 2:] The desired joint position $\mathbf{q}_d(t)$ is computed by solving inverse kinematics.
% 	%	, i.e., $\mathbf{h}_c(\mathbf{q}_d(t)) - \mathbf{h}_d(t,\theta_d) =\mathbf{0}$.
% 	\item[Step 3:] $\mathbf{q}_d$(t) is fed into the joint controllers, which emulate the \YanMod{default} joint controllers of a physical OP3 robot.
% \end{itemize}
% {A flow chart of the procedue is shown in Fig.~\ref{flow}.}
